Distributed Ensembles of Reinforcement Learning Agents for Electricity Control

Deep Reinforcement Learning (or just "RL") is gaining popularity for industrial and research applications. However, it still suffers from some key limits slowing down its widespread adoption. Its performance is sensitive to initial conditions and non-determinism. To unlock those challenges, we propose a procedure for building ensembles of RL agents to efficiently build better local decisions toward long-term cumulated rewards. For the first time, hundreds of experiments have been done to compare different ensemble constructions procedures in 2 electricity control environments. We discovered an ensemble of 4 agents improves accumulated rewards by 46%, improves reproducibility by a factor of 3.6, and can naturally and efficiently train and predict in parallel on GPUs and CPUs.

==> app.tex <==
\subsection{Note on the continuous combination rule}
\label{app:combi}

Weighted averaging predictions may not suit all RL applications with continuous action space.

Imagine the intuitive situation where an autonomous vehicle is driven with an ensemble of RL agents with continuous action space to control the wheel. When the car is approaching a crossroad it is facing multiple roads with physical constraints between each roads. When base agents disagree and interpolate their trajectories, the ensemble would hit physical constraints. This simple example shows that the combination rule should be designed by taking into account the specificity of the domain application. In our simulators, there is no such physical constraint between two continuous actions.

To better generalize on all simulators we propose the combination rule ``the closest base predictions to the weighted averaging''. When a new state is incoming, it computes the continuous action in 2 steps:
\begin{enumerate}
    \item Compute the weighted averaging $\hat{p}$ from all base predictions $P$ and weights $W$.
    \item Return the closest base predictions to $\hat{p}$ in $P$. We used the Euclidean distance.
\end{enumerate}

All base predictions are used to compute an agreement and elect the base prediction. It achieves two main properties. First, the ensemble prediction matches one single RL base agent's predictions that is previously trained to avoid the constraints of the environment. Second, all base agents contribute to computing the weighted averaging and may stabilize the final prediction.

We do not perform experiments on other RL applications to limit our studies to electricity control applications. We performed hundreds of hyperparameters sampling on both Pymgrid and GEM and observed no significant gain or loss using this combination rule compared to the weighted averaging.









%Three base agents answering respectively -30° -30° and +30° averaging their predictions would return +10°. A simple averaging of the predictions would drive the autonomous car in the wall which is an unwanted action.





% We propose a new combination rule
% \begin{algorithm}[Closest predictions to the averaging]
% \caption{}
% \label{algo:speed}
% \begin{algorithmic}[1]

% \STATE{\textbf{input:} $P$ predictions, $W$ weights}
% \STATE{\textbf{output:} The combined prediction $p\_ens$}
% \STATE{\textbf{start}}

% \STATE{\\ computed the standard weighted averaging}
% \STATE{avg $\gets$ $P*w$}


% \STATE{dist $\gets$ }


% \STATE{ $A\_speed$ $\gets$ bench($A$,$calib\_data$)}
% \STATE{$iter$ $\gets$ 0}

% \WHILE{$iter < max\_iter$}

% \STATE{$neighs$  $\gets$ neighborhood($A$) }
% \IF{length($neighs$) $>$ $max\_neighs$}
% \STATE{$neighs$  $\gets$ draw randomly $max\_neighs$ samples from $neighs\_A$ }
% \ENDIF

% \STATE{$best\_A$, $best\_speed$  $\gets$ for all $n$ in $neighs$ return the best one and its score based on the bench($n$,$calib\_data$) criterion }
% \IF{$best\_speed > A\_speed$}
%     \STATE{$A$ $\gets$ $best\_A$}
%     \STATE{$A\_speed$ $\gets$ $best\_speed$}
%     \STATE{$iter$ $\gets$ $iter$ + 1}
% \ELSE
%     \STATE{// local maxima (or plateau) detected}
%     \STATE{$iter$ $\gets$ $max\_iter\_greedy$}
% \ENDIF


% \ENDWHILE

% \STATE{return  $A$}

% \end{algorithmic}

% \end{algorithm}
